Utilization of Impedance Disparity Incurred from Switching Activities to Monitor and Characterize Firmware Activities

The massive trend toward embedded systems introduces new security threats to prevent. Malicious firmware makes it easier to launch cyberattacks against embedded systems. Systems infected with malicious firmware maintain the appearance of normal firmware operation but execute undesirable activities, which is usually a security risk. Traditionally, cybercriminals use malicious firmware to develop possible back-doors for future attacks. Due to the restricted resources of embedded systems, it is difficult to thwart these attacks using the majority of contemporary standard security protocols. In addition, monitoring the firmware operations using existing side channels from outside the processing unit, such as electromagnetic radiation, necessitates a complicated hardware configuration and in-depth technical understanding. In this paper, we propose a physical side channel that is formed by detecting the overall impedance changes induced by the firmware actions of a central processing unit. To demonstrate how this side channel can be exploited for detecting firmware activities, we experimentally validate it using impedance measurements to distinguish between distinct firmware operations with an accuracy of greater than 90%. These findings are the product of classifiers that are trained via machine learning. The implementation of our proposed methodology also leaves room for the use of hardware authentication.

==> Lit_Review.tex <==
%PDNPulse: Sensing PCB Anomaly with the Intrinsic Power Delivery Network - by H. Zhu, et al
%    This paper explains the results of detecting Hardware Trojans using a VNA through the power distribution network. This paper focused on the analyzing the impedance of the PCB to detect physical anomalies in the board (recycled PCBs, malicious components, counterfeit processors, etc.) Their method used the Frechet between a standard circuit frequency and an anomalous frequency response. 

%STELLAR: Generic EM SCA Protection through Root-Cause Analysis: D. Das. M. Nath, B. Chaterjee, et al
%    This paper dedicates half of its contents to discussing why chips emit EM radiation. The CPU tells the CMOS Logic gates to change state. This change in logic states causes some change in current. The current travels through the various etched metallic layers in the chip. The minuscule distances between these contacts causes radiation to unintentionally be radiated in the UHF an SHF frequencies (1 GHz to 10 GHz). Due to this range of frequencies of these emissions and the relation between EM and power, monitoring a pin may be able to reveal some of the inner workings of an embedded system.
    
A Review of Anomaly Detection Techniques Leveraging SCA - D. Spatz, D. Smarra, I. Ternovsky
    ML Algorithms are essential for processing the large volumes of SC emissions. Refined Feature Identification  are crucial to detect meaningful features from the large amounts of data. 

%Preliminary Classification of Results of RF Emission based Feature Extraction in IOT Devices  - D. Spatz, D. Smarra, I. Ternovsky
%    This paper states the effectiveness of the Frequency Domain in analyzing a Power signal. After transforming each collected signal, they divided the frequency-data into frequency bins and  calculated the mean and variance of each bin. 

%Obfuscation Revealed: Leveraging Electromagnetic Signals for Obfuscated Malware Classification: D. Pham, D. Marion, M. Mastio, A Heuser
%    By collecting data with a near-field RF Probe, researchers revealed were able to detect Malware running on an IoT device by taking a time-domain signal and classifying the collected data based on the spectrum of frequencies. 

%Toward an RF  Side Chanel Reverse Engineering Tool - M. Wilt, M. Baker, S. Papdakis
%    This paper showed that through collecting EM radiation, a machine learning classifier was able to detect the OS and even the software being run on a computer with high accuracy.

On the Limits of EM based Detection of Control Logic Injection Attacks
    Majority of research surrounding EM based analysis is extremely dependent on noise reduced environments. The research ignores the implications of real-life situations.
    This work finds that malicious code pollutes the intended execution code. Using 

